Towards Ordinal Data Science

Order is one of the main instruments to measure the relationship between objects in (empirical) data. However, compared to methods that use numerical properties of objects, the amount of ordinal methods developed is rather small. One reason for this is the limited availability of computational resources in the last century that would have been required for ordinal computations. Another reason -- particularly important for this line of research -- is that order-based methods are often seen as too mathematically rigorous for applying them to real-world data. In this paper, we will therefore discuss different means for measuring and 'calculating' with ordinal structures -- a specific class of directed graphs -- and show how to infer knowledge from them. Our aim is to establish Ordinal Data Science as a fundamentally new research agenda. Besides cross-fertilization with other cornerstone machine learning and knowledge representation methods, a broad range of disciplines will benefit from this endeavor, including, psychology, sociology, economics, web science, knowledge engineering, scientometrics.

==> sec-data-archaeology.tex <==
\section{Ordinal Data Science as Specific Approach to Data Archaeology}

\todo{Der folgende Text ist  aus [Hereth, J., Stumme, G., Wille, R., Wille, U.: Conceptual Knowledge Discovery - a Human-Centered Approach Journal of Applied Artificial Intelligence (AAI). 17, 281–301 (2003). \cite{hereth03conceptual}] kopiert und muss noch gekürzt werden.} 

According to R. S. Brachman and T. Anand (1996), much attention and effort in the field of KDD has been focused on the development of data-mining techniques, but only a minor effort has been devoted to the development of tools that support the analyst in the overall discovery task. They see a clear need to emphasize the process-orientation of KDD tasks and argue in favor of a more human-centered approach for a successful development of knowledge-discovery support tools (see also Uthurusamy 1996,p. 564). All in all, human-centered KDD refers to the constitutive character of human interpretation for the discovery of knowledge, and stresses the complex, interactive process of KDD as being lead by human thought.In practice, knowledge-discovery applications, obviously, vary in terms of underlying data, complexity, the amount of human involvement required,and their degree of possible automation of parts of the discovery process. In most applications, however, an indispensable part of the discovery process is that the analyst explores the data and sifts through the raw data to become familiar with it and to get a feel for what the data may cover. Often an explicit specification of what one is looking for only arises during an interactive process of data exploration, analysis, and segmentation. 

R. S. Brachman et al. (1993) introduced the notion of Data Archaeology for KDD tasks in which a precise specification of the discovery strategy, the crucial questions, and the basic goals of the task have to be elaborated during such an unpredictable interactive exploration of the data. Data Archaeology can be considered a highly human-centered process of asking, exploring, analyzing,interpreting, and learning in interaction with the underlying database. A human-centered approach to KDD that supports the overall KDD process should be based on a comprehensive notion of knowledge as a part of human thought, rather than on a restrictive formalization as it is used for the evaluation of automated knowledge-discovery or data-mining findings(for example, Fayyad et al. 1996, p. 8). The landscape paradigm of knowledge underlying Conceptual Knowledge Processing as described in Wille (1997) provides such a comprehensive and human-centered notion of knowledge. Although there is some similarity with the archaeology metaphor, the landscape paradigm places more emphasis on the intersubjective character of knowledge. Following Peirce’s pragmatic philosophy, knowledge is understood as always being incomplete, formed and continuously assured by human argumentation within an intersubjective community of communication (Wille 1997; Wille 2002). Knowledge discovery based on such an understanding of knowledge should support knowledge communication as a part of the KDD process, both with respect to the dialog between user and system and also as a part of human communication and argumentation. 

This presupposes a high transparency of the discovery process and a representation of its (interim) findings that support human argumentation to establish intersubjectively assured knowledge. Further fundamental requirements for human-centered KDD support tools have been stated by R. S. Brachman and T. Anand (1996,p. 53). In addition to tools that support the individual phases of the KDD process, they basically demand support for the coupling of the overall process, for exploratory Data Archaeology, and some help in deciding what discovery techniques to choose. Most of the content of these claims is covered by the more explicit and detailed requirements formulated already in (Brachman et al. 1993). Requirements 1 to 5 of the subsequent list are explicitly stated in (Brachman et al. 1993, p. 164), while the remaining requirements are implicit in (Brachman and Anand 1996; Brachman et al. 1993).



Noch erwähnen/zitieren: 

Was hat das mit Ordnungen/FCA zu tun?

Datenanalyse für Jedermann

 Stumme, G.: Off to New Shores -- Conceptual Knowledge Discovery and Processing Intl. J. Human-Comuter Studies (IJHCS). 59, 287–325 (2003).
 \cite{stumme03off}
 

Hereth, J., Stumme, G., Wille, R., Wille, U.: Conceptual Knowledge Discovery - a Human-Centered Approach Journal of Applied Artificial Intelligence (AAI). 17, 281–301 (2003). \cite{hereth03conceptual}


==> sec-genesis_of_ordinal_data.tex <==
\section{Genesis of ordinal data}

There exists a large variety of natural and social processes that generate ordinal data. Each type of process is producing ordered sets with specific characteristics, which have to be coped with when analysing the data \fuehrtzu{RA\,3, 4 \& 5}. Two categories of order generating processes can be identified: intrinsic relational and extrinsically induced.
\randbemerkung{Intrinsic relational orders}%
\fett{Intrinsic relational orders} arise from establishing an order relation between two individual entities. Typical examples are the parent/child relation between human beings, the (direct or indirect) citation of one publication by another, or the organization of conceptual knowledge in taxonomies (ontologies/concept hierarchies). In this case, the established relation does not (necessarily) depend on other properties of the involved entities. 
\mainobjective%
This kind of data is challenging for an analysis, as there exists a priori no easy way to break down the dataset to meaningful subsets based on the order relation \fuehrtzu{RA\,3, RA\,4}.
\randbemerkung{Extrinsicly induced orders}
\fett{Extrinsicly induced orders} result from features of the entities which can be used for their comparison. A prominent case are numerical valuations, \eg by size and prize, as described at the beginning of Section~\ref{subsub-historical}. These benefit from the interval (or ratio) level of measurement, and allow thus for measures of tendency such as mean and variance. 
\mainobjective%
For analysing the compatibility of orders and metrics and exploring joint representations, we will introduce \fett{metric ordered spaces (mo-spaces)} \fuehrtzu{RA\,2} in analogy to \emph{metric measure spaces}.
\randbemerkung{Predefined scales}
Not all extrinsicly induced orders are numerically induced.  For specific applications such as seismic activity or the hardness of minerals, there exist \fett{standard} (linear) \fett{ordinal scales} \footnote{see \url{https://de.wikipedia.org/wiki/Liste_ordinaler_Skalen}}. Otherwise, (\eg in psychological surveys or judgements in scientific peer reviewing), frequently 5- or 7-point Likert scales are used.
It is this kind of ordinal scales (in Stevens' original meaning) for which the current state of the art of RTM already provides an answer to the question under which conditions a measurement exists.

\randbemerkung{Boolean attributes induce orders}
Another frequently found type of ordinal data arises from \fett{Boolean attributes} such as `has two legs' or `is serving airports in Africa'. Even though the resulting linear scale (objects having the attribute are `better equipped than' those not having it) is of modest size 2 only,
\randbemerkung{Exponential explosion}%
the number of potential combinations 
grows exponentially (in the worst case, when there are no dependencies in the data) with the number of attributes, which may be extremely large. Consider, for instance, the bag-of-words model in information retrieval, where each word in the vocabulary provides one such binary attribute, and where vocabularies may rise easily to millions (e.g., the ClueWeb09~\cite{callan2009clueweb09} dataset of 500\,M web pages exhibits a vocabulary size of 38\,M). 
\mainobjective%
Thus, guidance is required for splitting \fuehrtzu{RA\,3} and reducing \fuehrtzu{RA\,4} large ordinal data into manageable parts and for navigating in the collection of these parts \fuehrtzu{RA\,5}.

\randbemerkung{Formal Concept Analysis}
In the field of \fett{Formal Concept Analysis}~(\cite{wille82restructuring}, \cite{ganter99formal}, \selfcite{ganter05formal}), a rich body of mathematical results has been built up for this type of data. In particular, it provides algebraic methods for decomposing large ordered sets into smaller ones. Unfortunately, most of the real-life ordered sets do not completely fulfil the structural requirements needed for the decompositions. 
\mainobjective%
What is missing in this respect are methods for decompositions, even if the data are noisy or contain some exceptions. The development of such methods  \fuehrtzu{RA\, 3} is particularly challenging, because there exists up to now no methodology dealing with \fett{local disruptions} of algebraic structures, because this is not in the spirit of research in the field of \fett{universal algebra}.


\randbemerkung{Combinations of orders}
The described combination of the 2-element-scales derived from binary attributes is just a specific case of combining different orders to one all-encompassing order. This approach is equivalent to $\mathbb{R}^n$ in the numerical case, as mentioned in Section~\ref{subsub-historical}, and can be applied to heterogeneous ordered sets. In scientometrics, for instance, on a collection of publications, one typically considers the citation hierarchy ($p_1\leq p_1$ if paper $p_2$ cites paper $p_1$ directly or there exists a chain of citing papers between them) together with a hierarchy derived from the bag-of-words model of the words in the abstract and with a hierarchy derived from the \texttt{author}-relation between publications and authors. 
\mainobjective%
As these hierarchies come with different characteristics, hybrid methods for exploring heterogeneous datasets have to be developed \fuehrtzu{RA\,5}.


\fett{In ORDER, we will focus on the development of data science methods for ordinal data, as they lack the large variety of methods that have been developed for numerical data.} The new methods will allow discovering and explain new structures and dependencies in ordinal data, and to efficiently explore large, heterogeneous collections of ordinal data.







==> steinbruch.tex <==
\section{Steinbruch}
Material aus dem ERC-Antrag etc., das ggf. noch ausgeschlachtet werden kann:














